Strategies for on-chip digital data compression for X-ray pixel detectors

The continued desire for X-ray pixel detectors with higher frame rates will stress the ability of application-specific integrated circuit (ASIC) designers to provide sufficient off-chip bandwidth to reach continuous frame rates in the 1 MHz regime. To move from the current 10 kHz to the 1 MHz frame rate regime, ASIC designers will continue to pack as many power-hungry high-speed transceivers at the periphery of the ASIC as possible. In this paper, however, we present new strategies to make the most efficient use of the off-chip bandwidth by utilizing data compression schemes for X-ray photon-counting and charge-integrating pixel detectors. In particular, we describe a novel in-pixel compression scheme that converts from analog to digital converter units to encoded photon counts near the photon Poisson noise level and achieves a compression ratio of $>\!1.5\times$ independent of the dataset. In addition, we describe a simple yet efficient zero-suppression compression scheme called ``zeromask'' (ZM) located at the ASIC's edge before streaming data off the ASIC chip. ZM achieves average compression ratios of $>\!4\times$, $>\!7\times$, and $>\!8\times$ for high-energy X-ray diffraction, ptychography, and X-ray photon correlation spectroscopy datasets, respectively. We present the conceptual designs, register-transfer level block diagrams, and the physical ASIC implementation of these compression schemes in 65-nm CMOS. When combined, these two digital compression schemes could increase the effective off-chip bandwidth by a factor of 6-12$\times$.

==> edgecomp.tex <==

\subsection{Compression at the detector ASIC edge}
\label{sec:edge-compression}

The in-pixel encoding scheme described above makes no assumptions about the nature of the data measured by the detector. However, we can exploit redundancies in the data to further compress the data. In this section, we describe a lossless compressor located at the ASIC edge that exploits the most common redundancy in X-ray data---the zeros. The aim of lossless compression is to reduce data by identifying and eliminating statistical redundancy. The characteristics of input data affect both the complexity of the design and the compression ratio. In general, complex designs require significant effort to validate and test in an ASIC. Our goal is to identify a simple design that fulfills two requirements. 
%high compression ratios and stall-free operation. 
First, it must yield reasonably high compression ratios for typical X-ray datasets.  Second, operation must be stall-free; it must process input pixel data shifted from the pixel array every single clock cycle without causing any stall clock cycle or dropping any data. The design should also be simple and have a minimal resource footprint on the pixel detector ASIC with no dependency on any external IP libraries, which also reduces the ASIC validation and testing efforts dramatically.


\subsubsection{Analysis of four typical X-ray datasets}
We have analyzed four typical X-ray datasets from a third-generation storage ring light source to guide the design of the edge compressor. The first dataset is typical of high-energy X-ray diffraction (XRD) experiments of polycrystalline materials; the data consist of 300 images from a time-resolved additive manufacturing experiment at the Advanced Photon Source, APS 1-ID-E, taken with a Dectris Pilatus3 X CdTe 2M detector. The second dataset is typical of a ptychography  experiment; the data consist of 1,737 images from a ptychography experiment at APS 2-ID-D taken with the Dectris Eiger X 500K detector. The third and fourth datasets consist of typical X-ray photon correlation spectroscopy (XPCS) experiments with concentrated and dilute samples of polymer spheres diffusing in glycerol; the data consist of 1,000 images taken at APS 8-ID-I with the X-Spectrum Lambda 750K detector. Figure \ref{fig:x-ray-data} shows a single image from each dataset. All three datasets were taken with photon-counting detectors that we use to emulate a charge-integrating detector and have been digitally denoised as described in Section~\ref{sec:denoising}. As one can see, the majority of pixels in all the images are zero. Table~\ref{table:zero} includes a statistical analysis of the high-energy XRD, ptychography, XPCS concentrated, and XPCS dilute datasets on the zero-valued pixels and a compression ratio that gzip offline compression can achieve as a reference. The percentage of zero-valued pixels is calculated every frame. The mean, standard deviation, minimum, and maximum are calculated from the percentage of zero-valued pixels of all frames. As the brightness of upgraded storage ring light sources increases, the percentage of zero-valued pixels may decrease. However, new X-ray sources will allow scientists to study more weakly scattering samples with higher frame rate detectors, so the percentage of zero-valued pixels may stay the same or decrease. The four X-ray datasets have a wide range of zero-valued pixels that enable us to explore the limits of our streaming edge compressor.  The compression ratio of the gzip offline compressor, which employs Lempel-Ziv coding (LZ77), is obtained from the ratio between the original file size and the compressed file size of a dataset.


\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c||c|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} &
  %\begin{tabular}[c]{@{}c@{}}Mean\\\[\%\]\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean\\ \% \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Std Dev\\ \% \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Minimum\\ \% \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Maximum\\ \% \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}offline gzip\\compression ratio\end{tabular} \\ \hline
High-energy XRD   & 83.42 & 2.49 & 68.96 & 85.03  & 19 \\ \hline
Ptychography      & 97.42 & 0.23 & 96.2 & 97.77  & 70 \\ \hline
XPCS concentrated & 98.62 & 0.03 & 98.02 & 98.68  & 67 \\ \hline
XPCS dilute       & 99.9 & 0.01 & 99.8 & 99.91  & 351 \\ \hline
\end{tabular}
\caption{Statistics of zero-valued pixels per frame and offline software-based compressor results.}
\label{table:zero} 
\end{center}
\end{table}


\begin{figure}[htbp]
\centering 
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/4-dataset-images.pdf}
\caption{Four representative images for the (a) high-energy XRD, (b) ptychography, (c) XPCS concentrated, and (d) XPCS dilute datasets. Pixel values equal to zero are displayed in black and $\geq\!1$ in white. Note that the ptychography dataset taken with the Eiger 500K has been cropped to $558 \times 514$ pixels.}
\label{fig:x-ray-data} 
\end{figure}

\subsubsection{Design encoding scheme}
Since the majority of pixels in all the datasets are zero-valued pixels, a
natural thought is to employ run-length encoding (RLE) \cite{RLE},
which leverages the consecutiveness of the same value in the input sequence.
As a concrete example, an input sequence [2, 0, 0, 0, 0, 0, 0, 0] would be encoded into [1, 2, 7, 0] using one pixel storage (e.g., 9 bits) for the number of the occurrences of a pixel value and another pixel storage for the pixel value itself. In this example, the compression ratio is $2$.
Theoretically, as the length of the input sequence increases, the compression ratio increases.  According to the percentage of zero-valued pixels in Table~\ref{table:zero}, approximately 5 out of 6 pixels,
38 out of 39 pixels, 71 out of 72 pixels, and 999 out of 1,000 pixels are a zero-valued pixel in high-energy XRD, ptychography, XPCS concentrated, and XPCS dilute, respectively, thus allowing us to estimate the length of continuous zero-valued pixels. If 5 out of 6 pixels are continuous (the best case), four pixels are needed to encode 6 pixels, which yields $1.5\times$ in the compression ratio on high-energy XRD. Applying the same calculation to XPCS dilute, which has the highest percentage of zero-valued pixels, the theoretically possible maximum compression ratio would be $250\times$.
% $9.75\times$, $18\times$ and  for ptychography, XPCS concentrated 
However, zero values typically are distributed nonuniformly  through an X-ray image, which leads to higher variability in compression ratios. In the worst case for RLE, the output size is twice  the input size. Such higher variability in the encoded data size imposes a significant challenge to hardware design when it comes to I/O handling and can possibly be a source of stall. Thus we need an encoding scheme whose encoded data have little variability in the encoded data size.
%Although RLE yields a very high compression ratio particularly for XPCS, its compression ratio varies significantly depending on input data.

In this paper, we propose a new compression encoding scheme named ``zeromask'' (ZM) that compresses data by leveraging zero pixels. Figure~\ref{fig:zme} depicts how ZM encodes input data with an example. The output of ZM consists of metadata and non-zero-valued pixels, where the metadata are a sequence of bits that preserves the original position of zero and nonzero pixels in the input segment. Unlike RLE, this approach does not require zero pixels to be contiguous and is thus effective with a more random input as long as it contains zero pixels. To simplify the logic, we repurpose a pixel storage for the metadata.  With 9-bit pixel storage, it can hold a metadata for up to 9 pixels. Since the size of pixel arrays is generally bound to the power of 2 (e.g., 256x256), a reasonable choice for the number of input pixels (N) to each ZM compressor logic would be 8 instead of 9.
%considering that the number of the pixels in a pixel array is the power of 2.
The maximum length of the encoded data will be $N + 1$ when all pixels are nonzero; this yields the worst compression ratio ($0.88\times$ with N=8), which outperforms RLE with $0.5\times$ compression ratio; the minimum length of encoded data being one, which  includes only metadata,  yields the best compression ratio ($8\times$ with N=8).

\begin{figure}[htbp]
\centering
\includegraphics[width=.8\textwidth,origin=c,angle=0]{Figures/zme.eps}
\caption{Zeromask encoding scheme.}
\label{fig:zme} 
\end{figure}


An obvious restriction of ZM is that the maximum compression ratio is limited by the number of input pixels and the number of bits per pixel, which is equal to the number of bits per metadata. To relax this restriction, we employ a bit-shuffling operation that can effectively increase the input size by shuffling bits (Figure~\ref{fig:bitshuffle}); the operation  greatly resembles \textit{BitShuffle}~\cite{Bitshuffle}, a software implementation of a bit-level transpose operation. We denote the original input by $p(i)_j$, where i is the index of the pixel and j is j\ts{th} bit. The bit-shuffling operation simply converts $p(i)_j$ to $q(j)_i$. This operation resembles a matrix transpose and is reversible and thus decodable. 
With a 9-bit pixel, it converts 16 input pixels to 9 16-bit integer blocks.
%9 pixels with 16-bit resolution, 
%which is large enough for metadata.
The bit-shuffling operation is simply a set of wires between the input bits and the output bits in a correct order and requires no logic circuit in ASIC; hence it is inexpensive to implement and verify.
After the bit shuffling, we can simply use ZM to compress data. No redesign of ZM is needed; only the parameters need to be changed. The bit shuffling is effective for the X-ray datasets, particularly high-energy XRD, where a majority of nonzero pixels use only the lower bits such as the pixel value 1--4 or three least-significant bits. For example, a sequence of 9-bit input pixels [1, 2, 3, 1, 0, 2, 3, 1] is converted to a sequence of 9 integer blocks [179, 68, 0, 0, 0, 0, 0, 0, 0], where each integer block is 8 bits.\footnote{The decimal number 179 is 10110011 in binary, and 68 is 01000100.}

\begin{figure}[htbp]
\centering
\includegraphics[width=.6\textwidth,origin=c,angle=0]{Figures/bitshuffle.eps}
\caption{Bit-shuffling scheme.}
\label{fig:bitshuffle} 
\end{figure}

To evaluate different encoding schemes, we also developed a software tool\footnote{The tool is written in Scala so that we can reuse codes in Chisel testbenches to verify the outputs from simulated hardware.} that reads actual X-ray datasets from a file and compresses input data by using different encoding schemes. Each dataset frame is divided by eight or sixteen rows, depending on the input size to the encoder.  For example, with the XPCS datasets ($1556\times512$ pixels), each frame is broken into 64 chunks with eight input pixels and 32 chunks with sixteen input pixels, where each chunk has 1,556 columns. Columns in each chunk are fed into encoders one by one,  emulating the shift operation of the pixel array. It iterates the same process for all chunks in each frame. We evaluate the compression ratio of all frames in all four X-ray datasets. The compression ratio is calculated by dividing the total number of the input pixels per frame by the total number of the encoded pixels.  Tables \ref{table:crxrd}, \ref{table:crpty}, \ref{table:crxpcsc},  and \ref{table:crxpcsd} show the compression ratios obtained on the four datasets with different encoding schemes as well as statistics of the variation across all the images in each dataset. The bit width of input pixels is 9 bits.
Of  the three encoding schemes (run-length, zeromask, and shuffled zeromask),
the shuffled zeromask scheme achieves the highest compression for all four datasets and the lowest relative standard deviation. Moreover,  the zeromask scheme achieves the second best compression ratio with a comparatively lower relative standard deviation. 
% New paragraph here?
Earlier in Table~\ref{table:zero} the gzip compression ratios for the four datasets were presented and are significantly larger than shuffled zeromask. However, that gzip compression was performed on the entire dataset. If gzip is used over a smaller dataset, its performance is severely degraded. We have also evaluated the compression of gzip on smaller input sizes. We compressed 8 or 16 bytes input patterns (all zero or all different) using a Python gzip library, which internally uses the standard zlib library. The compression results shown in Table~\ref{table:smallgzip}  clearly indicate that gzip is inefficient for smaller input sizes.


%that encodes eight or sixteen input column pixels and packs variable-size encoded data into a buffer. 
% To simplify the coalescing logic, it inserts an encoded data to a buffer in the next clock cycle when its size exceeds the available space in the current buffer, thus there may be some unoccupied pixels in the buffer output, which affects the compression ratio.

\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Encoding}} &
  \begin{tabular}[c]{@{}c@{}}Input\\pixels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean \\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Std Dev\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Minimum\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Maximum\\ CR\end{tabular} \\ \hline
Run-length & 8 & 1.4 & 0.08 & 1.0 & 1.5 \\ \hline
Run-length & 16 &  1.6 & 0.11 & 1.0 & 1.7 \\ \hline
Zeromask & 8 &  3.5 & 0.23 & 2.3 & 3.6 \\ \hline
Shuffled zeromask & 16 & 4.2 & 0.13 & 3.5 & 4.3 \\ \hline
\end{tabular}
\caption{Compression ratios of various encoding schemes---high-energy XRD.}
\label{table:crxrd} 
\end{center}
\end{table}

\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Encoding}} &
  \begin{tabular}[c]{@{}c@{}}Input\\pixels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean \\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Std Dev\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Minimum\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Maximum\\ CR\end{tabular} \\ \hline
Run-length & 8 &  3.3 & 0.05 & 3.0 & 3.3 \\ \hline
Run-length & 16 &  5.4 & 0.14 & 4.7 & 5.6 \\ \hline
Zeromask & 8 &  6.6 & 0.10 & 6.1 & 6.7 \\ \hline
Shuffled zeromask & 16  & 7.3 & 0.07 & 6.9 & 7.4 \\ \hline
\end{tabular}
\caption{Compression ratios of various encoding schemes---ptychography.}
\label{table:crpty} 
\end{center}
\end{table}

\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Encoding}} &
  \begin{tabular}[c]{@{}c@{}}Input\\pixels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean \\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Std Dev\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Minimum\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Maximum\\ CR\end{tabular} \\ \hline
Run-length & 8 & 3.6 & 0.01 & 3.4 & 3.6 \\ \hline
Run-length & 16 & 6.4 & 0.03 & 5.9 & 6.4 \\ \hline
Zeromask & 8 & 7.2 & 0.02 & 6.9 & 7.2 \\ \hline
Shuffled zeromask & 16 & 8.3 & 0.02 & 8.0 & 8.4 \\ \hline
\end{tabular}
\caption{Compression ratios of various encoding schemes---XPCS concentrated.}
\label{table:crxpcsc} 
\end{center}
\end{table}

\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Encoding}} &
  \begin{tabular}[c]{@{}c@{}}Input\\pixels\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean \\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Std Dev\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Minimum\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Maximum\\ CR\end{tabular} \\ \hline
Run-length & 8 &  4.0 & 0.002 & 3.9 & 4.0 \\ \hline
Run-length & 16 &  7.8 & 0.01 & 7.6 & 7.8 \\ \hline
Zeromask & 8 &  7.9 & 0.003 & 7.87 & 7.94 \\ \hline
Shuffled Zeromask & 16 &  8.9 & 0.004 & 8.8 & 8.9 \\ \hline
\end{tabular}
\caption{Compression ratios of various encoding schemes---XPCS dilute.}
\label{table:crxpcsd} 
\end{center}
\end{table}


\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Input Size}} &

  \begin{tabular}[c]{@{}c@{}}Best\\ CR\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Worst\\ CR\end{tabular}  \\ \hline
8  &  0.35 &  0.29   \\ \hline
16 &  0.70 &  0.44  \\ \hline
\end{tabular}
\caption{Small input sizes with gzip.}
\label{table:smallgzip} 
\end{center}
\end{table}


% Here, we explore a zero-suppression logic that uses a 256-bit output bus. The 256-bit output bus can hold 28 pixels, which can hold 3 worst case encoding data.  We need to take into account I/O constraints if the bit width to peripheral devices (e.g., SRAM block, network interface) is fixed. Since the encoded data are variable in length, how to pack variable-size data into a fixed size output is key in the design.

\subsubsection{Design methodology using Chisel}

Before we describe the design and implementation of the streaming edge compressor, we describe our design methodology.
%The implementation of complex compression algorithms is not necessarily straightforward on digital logic (i.e., Verilog).
To improve both the productivity and quality of digital circuit designs, 
%leveraging the power and flexibility of the emerging hardware design language named Chisel \cite{Bachrach:ft},
we have designed and implemented a hardware compressor generator framework (Figure \ref{hacogen}) that generates a concrete compressor RTL design.

Our compressor design is highly parameterized and fully written in the emerging hardware design language Chisel \cite{Bachrach:ft} so that it can generate a wide range of hardware configurations (e.g., different numbers of input/output pixels and bit widths and eventually different compressor algorithms). The framework not only provides a mechanism to generate synthesizable Verilog codes of a streaming compressor with specified design parameters such as input/output sizes and  bit width; it also provides a fully integrated, flexible test harnesses and a test pattern generator that allows us to test the compressor design with various test patterns before Verilog is synthesized and implemented in a particular ASIC technology node. 

\begin{figure}[htbp]
\centering 
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/Fig_Framework.pdf}
\caption{Hardware compressor generator framework.}
\label{hacogen} 
\end{figure}

Chisel is rapidly gaining popularity in digital circuit design and has been used in various ASIC and FPGA projects. A notable project based on Chisel is the Rocket Chip generator \cite{Asanovic:EECS-2016-17}, which has generated RISC-V processor RTL designs with several tape-outs. Chisel is an open-source hardware construction language, implemented as class libraries of the Scala language. With the power of Scala, a modern functional, object-oriented language, it allows designers to express complicated circuit blocks far more easily and more concisely than hardware description languages (HDLs) allow; this improves readability and reduces errors. The important characteristics of Chisel are zero-cost abstraction, higher level of expressibility, and controllability. Chisel is not a high-level synthesis tool. Chisel not only provides the abstraction of digital circuit primitives such as combinational logics, wires, registers, and memories  but also provides some basic structures such as multiplexer, first-in first-out, queue, and shift registers, which are defined in the Chisel standard library. Additionally, larger building blocks such as floating-point operations are available as open source. Chisel also includes fully integrated frameworks for unit tests so that developers can write unit tests in Scala, and it seamlessly integrates external Verilog simulators such as Verilator. More important, it is fairly easy to install and use; a simple command line invocation of Chisel will generate Verilog codes, run Scala testbenches, and invoke Verilator to generate a value change dump (VCD) file.

% removed listing and associated listing. per reviewer's request
% simply removing this paragraph is ok because this is not essential to the paper.
%Listings \ref{verilog} and \ref{chisel} show a comparison between Verilog and Chisel using a simple delay circuit. Although it is impossible to show the whole view of Chisel with a small example, this example renders some fundamental features in Chisel, compared to Verilog. First of all, the Chisel version has no clock, reset signals and \lstinline|always| blocks because it automatically infers clock and reset signals when needed. Since the default form of the state element provided by Chisel is a positive-edge register that supports synchronous reset, no \lstinline|always| blocks are needed. In this example, \lstinline|RegNext()| delays its input by one clock cycle and copies it to the output.  Such limitation in the state element enforces a design guideline transparently and makes Chisel syntax more concise at the cost of flexibility. Chisel provides frequently-used data types such as Int, UInt, Int, instead of a range of bits like in Verilog, which also improves readability.

%\begin{parcolumns}[nofirstindent]{2}
% \colchunk{
%  \noindent\begin{minipage}{.45\textwidth}

%\begin{lstlisting}[language=Verilog,caption=Simple delay circuit in %Verilog,label={verilog}]
%module delay(
%  input        clock,
%  input        reset,
%  input  [7:0] io_in,
%  output [7:0] io_out
%);
% reg [7:0] r0;
% reg [7:0] r1;
%assign io_out = r1;

%  always @(posedge clock) begin
%   r0 <= io_in;
%    r1 <= r0;
%  end
%endmodule
%\end{lstlisting}

 % \end{minipage}
 %}
 %\colchunk{
 % \begin{minipage}{.45\textwidth}

%\begin{lstlisting}[language=Scala, caption = Simple delay circuit in %Chisel, label={chisel},frame=single]
%class delay extends Module {
%    val io = IO(new Bundle {
%    val in  = Input(UInt(8.W))
%   val out = Output(UInt(8.W))
%  })
%  val r0 = RegNext(io.in)
%  val r1 = RegNext(r0)
%  io.out := r1
%}
%}
%\end{lstlisting}
%  \end{minipage}
% }
% \colplacechunks
%\end{parcolumns}

%removed; this paragraph was redundant.
%Chisel provides powerful Scala-based testbench frameworks. Designers leverage the power and feature of the modern general-purpose language to test their circuit designs.  All Scala libraries (I/O, math, statistical, etc.), for example, can be used to test their circuits. Chisel also invokes Verilator to generate C++-based fast cycle accurate simulators from Verilog codes generated by Chisel.

\subsubsection{Design of streaming edge compressor}
\label{sec:compressor-design}
The streaming edge compressor is a data compression logic between the pixel array and a peripheral logic such as a network interface or a memory. The two most important design considerations of the streaming compressor are being stall-free (i.e., deterministic with a fixed latency) and having a small resource footprint. Since the pixel array generates (column) pixel data at a fixed rate, the compression logic must process the data without any stall condition, which would cause data dropping. For this design we avoided inferring a large-enough memory for the compression logic to temporarily store pixel data because of two factors: (1) the length of each experiment, which determines the size of a temporary memory, is unknown, and (2) the resources (e.g., the number of transistors) are scarce on the detector ASIC chip.

Figure~\ref{fig:hwcomp} shows the basic architecture of the streaming edge compressor. The main part of the streaming compressor is the encoding stage, which is an implementation of the zeromask compressor. 
The coalescing stage is needed for fixed-size peripherals (such as SRAMs, memory controllers). The encoding stage generates encoded data every clock cycle. The size of the encoded data varies depending on the content of the input data. The coalescing stage packs these variable-sized encoded data fragments into an internal buffer whose size aligns with the data bus width of a target device before sending it to the target device.  The number of clock cycles required until the internal buffer becomes ready to be read is also variable.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/basic-comp.eps}
%\caption{\textbf{ Basic design of streaming edge compressor.}
\caption{Basic architecture of the streaming edge compressor}
\label{fig:hwcomp} 
\end{figure}

\paragraph{Encoding stage} The encoding stage receives column pixel data from the pixel array every clock cycle, performs the ZM encoding, and generates encoded data whose size is variable between 1 to (N+1), where N is the input size. 

Figure \ref{encodingstage} shows the basic idea of how the encoding stage generates an encoded data fragment. An encoded data fragment consists of a metadata header and a series of nonzero pixels; and the number of pixels encoded is chosen so that the metadata, a bit
field where a 0 bit encodes a suppressed pixel, fits a single pixel bit-length.
The metadata creation logic is basically a combination of comparators and bit-shift operations. Chisel allows such circuits to be expressed in a concise manner.
%where the metadata is designed to fit to a single pixel.
% For the ZM compressor logic, each bit field in the metadata is associated with each pixel, and each bit field indicates whether the associated pixel is non-zero or not.  For example, if the first pixel is non-zero, the first metadata bit field is set to one. If the third pixel is zero, the third bit field is set to zero.

\begin{figure}[htbp]
\centering 
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/packinglogic.eps}
\caption{Encoding stage: metadata creation and packing.}
\label{encodingstage} 
\end{figure}


%Listing \ref{chiselmetadata} includes the actual code used in our Chisel-based generator framework that generates the mask bits.
%The default parameters are defined in class parameters (\lstinline|npixels| is 8 and \lstinline|pixelbitwidth| is 9 in this example), which can be changed when the \lstinline|Header| class is instantiated. With the default parameters, the I/O block defines eight integer values (eight pixels) as input and a single integer (one pixel) as output. The \lstinline|VecInit.tabulate()| method creates a vector whose element is an integer that holds a mask value for each pixel. If a pixel is nonzero, the mask value is the left-shift of 1 by \lstinline|i|, where \lstinline|i| is the base index of the pixel (e.g., 1<<0 for the first pixel). If a pixel is zero, the mask value is simply zero. The metadata vector is then reduced into a single integer by an OR operation of each element to generate the metadata header.

%\begin{lstlisting}[language=Scala, caption = Metadata generation in %Chisel, label={chiselmetadata},frame=single]
%class Header(val npixels:Int = 8, val pixelbitwidth:Int = 9) extends %Module {
%    val io = IO(new Bundle {
%       val in  = Input(Vec(npixels, UInt(pixelbitwidth.W)))
%       val out = Output(UInt(pixelbitwidth.W))
%    })
%
%   val metadata = VecInit.tabulate(npixels)(i => (io.in(i) =/= 0.U).asUInt << i)
%   io.out := metadata.reduce(_ | _)
%}
%\end{lstlisting}

The rest of the encoding logic is the packing logic that removes zero pixels from the input pixel data, which includes both nonzero and zero pixels, and generates a sequence of pixel data only with nonzero pixels while preserving the order of the pixels. 
%(Figure \ref{packing})

% It outputs pixel data that is the same size as the input and the pixel index, the \lstinline|pos| indicators ?? position (\lstinline|pos|) indicators that holds the number of non-zero pixels. 

%\begin{figure}[htbp]
%\centering 
%\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/Fig_Packing.pdf}
%\caption{Packing sparse data into dense data.}
%\label{packing} 
%\end{figure}

Internally the packing logic consists of N copies of a logic named \lstinline|ShiftUp|. Each \lstinline|ShiftUp| logic receives pixel data (N pixels) and the \lstinline|pos| indicator that holds the index of the current pixel position. Then it outputs updated pixel data and \lstinline|pos| that holds the index of the pixel for the next logic. All \lstinline|ShiftUp| logics are sequentially connected; the outputs of the previous logic are connected to the inputs of the next logic, except the first and last logic. The input to the first \lstinline|ShiftUp| logic receives pixel data from the pixel array. The initial value of \lstinline|pos| is set to zero. The outputs from the last \lstinline|ShiftUp| logic are connected to the coalescing stage, which includes the pixel data that hold packed pixels and the position index that is equal to the number of the nonzero pixels.
%Listing \ref{packingcore} shows the core part of the packing logic. \lstinline|io.in()| is the input pixel data; \lstinline|io.pos| is the input pixel index; \lstinline|io.out()| is the output pixel data; and \lstinline|io.outpos| is the output pixel index. \lstinline|Mux()| is a multiplexer that selects the second argument when the first argument is true, or otherwise selects the third argument. The \lstinline|for| loop generates a conditional, partial shift logic that shifts all pixels above the current position when the current pixel is zero or connects the input pixel vector to the output pixel vector for all pixels whose index is below the current position.  The last pixel is filled with zero when it shifts.

%\noindent\begin{minipage}{\textwidth}
%\begin{lstlisting}[language=Scala, caption = The core part of packing %logic in Chisel, label={packingcore},frame=single]
%val sel = (io.in(io.pos) === 0.U)
%io.posout := Mux(sel, io.pos, io.pos + 1.U)
%for (i <- 0 to npixels - 2)  io.out(i) := Mux((i.U >= io.pos) & sel, %io.in(i+1), io.in(i))
%io.out(npixel - 1) := Mux(sel, 0.U, io.in(pixel - 1))
%\end{lstlisting}
%\end{minipage}

The number of lines in the entire packing logic is approximately 50, including boiler plate code, while the number of lines in the generated Verilog code is approximately 500 with \lstinline|npixel| = 8 and 1,600 with \lstinline|npixel| = 16. Note that the number of lines in the Chisel code stays the same for both configurations because it is fully parameterized. 

\paragraph{Coalescing stage} The data generated from the encoding stage are variable in size. If the interface of a peripheral device accepts variable-sized data, we can simply send encoded data into such a device. Otherwise, if the interface to the serializer expects a fixed size (e.g., 256 bits), a buffering mechanism is needed. The coalescing logic is a simple buffering logic that packs multiple variable-size encoded data into a fixed-size buffer before sending to the peripheral device.

The coalescing logic consists of two components: the \lstinline|Selector| and \lstinline|STBuf| module (see Figure \ref{coalescing}). The \lstinline|Selector| module receives the length of the encoded data every clock cycle from the encoding logic and updates the insert position (\lstinline|pos| in \lstinline|STBuf|) to the buffer in the \lstinline|STBuf| module of the associated encoded data. It raises the flushed signal when the buffer becomes full.  The \lstinline|STBuf| module receives \lstinline|flushed| and \lstinline|pos| from the \lstinline|Selector| module and the encoded data from the encoding stage and outputs the fixed-size data. It consists of an array of registers (buffer) and a barrel shifter.

\begin{figure}[htbp]
\centering 
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/coalescinglogic.eps}
\caption{Block diagram of the coalescing logic that packs encoded data into a fixed-size buffer.}
\label{coalescing} 
\end{figure}

\subsubsection{Verification}
All of the design components for the streaming ZM compressor are expressed in Chisel and are translated into Verilog codes. While we could simply use an external Verilog simulator such as ModelSim to verify the functionality of the generated Verilog codes, Chisel provides a fully integrated testing harness for functional verification that allows developers to write testbenches in Scala, instead of Verilog. It seamlessly invokes an external Verilog simulator (Verilator by default). Since Scala is a powerful general-purpose functional, object-oriented programming language, it allows one to write complex and flexible testbench codes.
%We verify the functionality of all subcomponents in the compressor design with their own unit test before integrating them into the entire compressor design.
In addition we have successfully verified the functionality of the entire compressor design (Figure \ref{testbench}) against all four X-ray datasets. The testbench reads data from actual datasets and uses the data as input  to the device under test (DUT) that runs a simulated streaming compressor. An image frame in a dataset is chunked up into N-row pixel strips, which are fed into DUT column by column. We iterate all frames in a dataset. For example, with N=16, a 256x256 image frame is chunked up to 16 strips,\footnote{Each strip is each compressor instance.} and each strip has 256 columns. The total encoding count per frame is 4,096 ($= 16 \times 256$) in this example.

\begin{figure}[htbp]
\centering
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/Fig_testbench.pdf}
\caption{Verification testbench.}
\label{testbench} 
\end{figure}

\subsubsection{Physical implementation}
Figure \ref{compressor-layout} shows examples of the described streaming compressors that were coded in RTL, synthesized, and placed and routed in \SI{65}{\nm} standard cell CMOS. Layout (a) shows a placed and routed 8-pixel ZM compressor.
The area of this block is close to the desired area of a single pixel, which means that an 8-pixel streaming compressor block could be located at the end of every pixel row with little impact on the ASIC floor plan. Placing one compressor per pixel row would add the equivalent area of a single column of pixels to the pixel array. Layout (b) shows a placed and routed 16-pixel ZM compressor. The area of this block would span two \SI{100}{\um} pixel rows. If one 16-pixel compressor block were placed at the end of every two pixel rows, it would add the equivalent area of 2 pixel columns to the pixel array.
Since the compressor block of layout (a) supports 8 pixel inputs, 8 parallel shift buses can be implemented per row, resulting in an 8-fold reduction in the row shift time.
Layout (c) shows a 16-pixel bit-shuffled ZM compressor. This version is slightly smaller than the non-shuffled example of (b). 
%Synthesis tool estimates the power consumption to be \SI{347}{\uW}, \SI{663}{\uW}, and \SI{635}{\uW} for the 8-pixel, 16-pixel, and bit-shuffled 16-pixel ZM compressors, respectively. These estimates do not include behavioral simulations of the switching activity. 

\begin{figure}[htbp]
\centering % \begin{center}/\end{center} takes some additional vertical space
\includegraphics[width=1\textwidth,origin=c,angle=0]{Figures/ANL-compressor-layouts5.pdf}
\caption{Physical layout of three variants of the ZM compressor in \SI{65}{\nm} CMOS: (a) 8-pixel, (b) 16-pixel,  and (c) 16-pixel bit shuffled.}
\label{compressor-layout} 
\end{figure}

